GL-GIN: Fast and Accurate Non-Autoregressive Model for Joint Multiple Intent Detection and Slot Filling

Multi-intent SLU can handle multiple intents in an utterance, which has attracted increasing attention. However, the state-of-the-art joint models heavily rely on autoregressive approaches, resulting in two issues: slow inference speed and information leakage. In this paper, we explore a non-autoregressive model for joint multiple intent detection and slot filling, achieving more fast and accurate. Specifically, we propose a Global-Locally Graph Interaction Network (GL-GIN) where a local slot-aware graph interaction layer is proposed to model slot dependency for alleviating uncoordinated slots problem while a global intent-slot graph interaction layer is introduced to model the interaction between multiple intents and all slots in the utterance. Experimental results on two public datasets show that our framework achieves state-of-the-art performance while being 11.5 times faster.

==> Related_Work.tex <==

\subsection{End-to-end Task-oriented Dialog}
\qlbcomment{we should add all related work here.}
End-to-end task-oriented dialog systems (ETODs) that adopt sequence-to-sequence (Seq2seq) model to achieve specific goals have attracted increasing attention, which can free from manually designed pipeline modules and can be easily adapted to a new domain.
Different seq2seq model on open-domain dialog, the successful conversations heavily rely on the accurate KB query.
Recently, 
\newcite{eric-etal-2017-key} performs attention over KB to generate entities.
\newcite{lei-etal-2018-sequicity} considers track dialogue believes in end-to-end task-oriented dialog.
\newcite{madotto-etal-2018-mem2seq} first combines end-to-end memory network \cite{DBLP:conf/nips/SukhbaatarSWF15} to consider KB query \cite{DBLP:conf/nips/SukhbaatarSWF15}.
\newcite{gangi-reddy-etal-2019-multi} proposes a multi-level memory architecture which first addresses queries, followed by results and finally each key-value pair within a result.
\newcite{DBLP:conf/iclr/WuSX19} proposes a global-to-locally pointer mechanism to query KB.
\newcite{qin2020dynamic} proposes a dynamic network to explicitly consider domain-shared and private features, which achieves state-of-the-art performance.
Compared with their models, our framework proposes a modularized pre-training framework to incorporate large amounts of unlabeled data. 

\subsection{Pre-training Models}
In recent yeas, GPT-based pre-trained model have been successfully adapted to various dialog tasks \cite{zhang-etal-2020-dialogpt,gong-etal-2020-tablegpt,peng-etal-2020-shot}.  
\newcite{zhang-etal-2020-dialogpt} proposes \texttt{DialoGPT} that further pre-trains on twitter dialog corpora for considering dialog features. 
\newcite{bao-etal-2020-plato} proposes a novel pre-training model for dialog generation,  incorporated with latent discrete variables for one-to-many relationship
modeling.
Different from their work, we focus on the task-oriented dialog domain.
Some work considers to adapt the GPT-2 model.
Besides,  pre-trained
language model like GPT-2 is also leveraged for modeling all pipeline sub-tasks dialogue state tracking, action and response generation as a single sequence in a unified way \cite{ham-etal-2020-end,yang2020ubar,hosseini2020simple} also receive growing attention, but are not within the scope of our discussion.
Compared with their work, we focus on the end-to-end TOD systems that directly
operate on dialog history and interact with knowledge base
without any intermediate supervision.
In addition, we further propose a novel modularized pre-training framework where two pre-training tasks to enhance the \textit{generation} and \textit{knowledge-retriever} module.
To the best of our knowledge, we are the first work to explore the pre-training method in end-to-end task-oriented dialog.
